Prompt Decoupling for Text-to-Image Person Re-identification

Text-to-image person re-identification (TIReID) aims to retrieve the target person from an image gallery via a textual description query. Recently, pre-trained vision-language models like CLIP have attracted significant attention and have been widely utilized for this task due to their robust capacity for semantic concept learning and rich multi-modal knowledge. However, recent CLIP-based TIReID methods commonly rely on direct fine-tuning of the entire network to adapt the CLIP model for the TIReID task. Although these methods show competitive performance on this topic, they are suboptimal as they necessitate simultaneous domain adaptation and task adaptation. To address this issue, we attempt to decouple these two processes during the training stage. Specifically, we introduce the prompt tuning strategy to enable domain adaptation and propose a two-stage training approach to disentangle domain adaptation from task adaptation. In the first stage, we freeze the two encoders from CLIP and solely focus on optimizing the prompts to alleviate domain gap between the original training data of CLIP and downstream tasks. In the second stage, we maintain the fixed prompts and fine-tune the CLIP model to prioritize capturing fine-grained information, which is more suitable for TIReID task. Finally, we evaluate the effectiveness of our method on three widely used datasets. Compared to the directly fine-tuned approach, our method achieves significant improvements.

==> tables.tex <==
\usepackage{subcaption}

\begin{table*}[ht]
  \centering  % 显示位置为中间
  \resizebox{0.9\textwidth}{!}{
  \begin{tabular}{l|clcc|ccccc}
  % \hline
  \toprule
  Method                                &Type &Ref     &Image Enc.&Text Enc.     &Rank-1            &Rank-5         &Rank-10        &mAP         &mINP                \\
  \hline
  \midrule
  % GNA-RNN\cite{li2017person}            &G    &CVPR17  &VGG       &LSTM          &19.05             &-              &53.64          &-              &-              \\
  % Dual Path\cite{zheng2020dual}         &G    &TOMM20  &RN50      &RN50          &44.40             &66.26          &75.07          &-              &-              \\
  CMPM/C\cite{zhang2018deep}            &L    &ECCV18  &RN50      &LSTM          &49.37             &-              &79.27          &-              &-              \\
  TIMAM\cite{sarafianos2019adversarial} &G    &ICCV19  &RN101     &BERT          &54.51             &77.56          &79.27          &-              &-              \\
  ViTAA\cite{wang2020vitaa}             &L    &ECCV20  &RN50      &LSTM          &54.92             &75.18          &82.90          &51.60          &-              \\
  NAFS\cite{gao2021contextual}          &L    &arXiv21 &RN50      &BERT          &59.36             &79.13          &86.00          &54.07          &-              \\
  DSSL\cite{zhu2021dssl}                &L    &MM21    &RN50      &BERT          &59.98             &80.41          &87.56          &-              &-              \\
  SSAN\cite{ding2021semantically}       &L    &arXiv21 &RN50      &LSTM          &61.37             &80.15          &86.73          &-              &-              \\
  LapsCore\cite{wu2021lapscore}         &L    &ICCV21  &RN50      &BERT          &63.40             &-              &87.80          &-              &-              \\
  ISANet\cite{yan2022image}             &L    &arXiv22 &RN50      &LSTM          &63.92             &82.15          &87.69          &-              &-              \\
  LBUL\cite{wang2022look}               &L    &MM22    &RN50      &BERT          &64.04             &82.66          &87.22          &-              &-              \\
  Han et al.\cite{han2021text}          &G    &BMVC21  &CLIP-RN101&CLIP-Xformer  &64.08             &81.73          &88.19          &60.08          &-              \\
  SAF\cite{li2022learning}              &L    &ICASSP22&ViT-Base  &BERT          &64.13             &82.62          &88.40          &-              &-              \\
  TIPCB\cite{chen2022tipcb}             &L    &Neuro22 &RN50      &BERT          &64.26             &83.19          &89.10          &               &-              \\
  CAIBC\cite{wang2022caibc}             &L    &MM22    &RN50      &BERT          &64.43             &82.87          &88.37          &-              &-              \\
  AXM-Net\cite{farooq2022axm}           &L    &MM22    &RN50      &BERT          &64.44             &80.52          &86.77          &58.73          &-              \\
  LGUR\cite{shao2022learning}           &L    &MM22    &DeiT-Small&BERT          &65.25             &83.12          &89.00          &-              &-              \\
  IVT\cite{shu2022see}                  &G    &ECCVW22 &ViT-Base  &BERT          &65.59             &83.11          &89.21          &-              &-              \\
  CFine\cite{yan2022clip}               &L    &arXiv22 &CLIP-ViT  &BERT          &\underline{69.57} &85.93          &91.15          &-              &-              \\
  \hline
  \textbf{Baseline (CLIP-RN50)}         &G    &-       &CLIP-RN50 &CLIP-Xformer  &57.26             &78.57          &85.58          &50.88          &34.44          \\
  \textbf{Baseline (CLIP-RN101)}         &G    &-       &CLIP-RN101&CLIP-Xformer  &60.27             &80.88          &87.88          &53.93          &37.54          \\
  \textbf{Baseline (CLIP-ViT-B/16)}     &G    &-       &CLIP-ViT  &CLIP-Xformer  &68.19  &\underline{86.47} &\underline{91.47} &\underline{61.12} &\underline{44.86}\\
  \textbf{IRRA (Ours)}                 &G    &-       &CLIP-ViT  &CLIP-Xformer  &\textbf{73.38} &\textbf{89.93} &\textbf{93.71} &\textbf{66.13} &\textbf{50.24}    \\
  % \hline
  \bottomrule
  \end{tabular}}%
  \caption{Performance comparisons with state-of-the-art methods on CUHK-PEDES dataset. Results are ordered based on the Rank-1 accuracy. ``G" and ``L" in ``Type" column stand for global-matching/local-matching method.}
  \label{tab:1}
  \vspace{-4mm}
  \end{table*}
